Evaluating the Potential of Disaggregated Memory Systems for HPC applications

Disaggregated memory is a promising approach that addresses the limitations of traditional memory architectures by enabling memory to be decoupled from compute nodes and shared across a data center. Cloud platforms have deployed such systems to improve overall system memory utilization, but performance can vary across workloads. High-performance computing (HPC) is crucial in scientific and engineering applications, where HPC machines also face the issue of underutilized memory. As a result, improving system memory utilization while understanding workload performance is essential for HPC operators. Therefore, learning the potential of a disaggregated memory system before deployment is a critical step. This paper proposes a methodology for exploring the design space of a disaggregated memory system. It incorporates key metrics that affect performance on disaggregated memory systems: memory capacity, local and remote memory access ratio, injection bandwidth, and bisection bandwidth, providing an intuitive approach to guide machine configurations based on technology trends and workload characteristics. We apply our methodology to analyze thirteen diverse workloads, including AI training, data analysis, genomics, protein, fusion, atomic nuclei, and traditional HPC bookends. Our methodology demonstrates the ability to comprehend the potential and pitfalls of a disaggregated memory system and provides motivation for machine configurations. Our results show that eleven of our thirteen applications can leverage injection bandwidth disaggregated memory without affecting performance, while one pays a rack bisection bandwidth penalty and two pay the system-wide bisection bandwidth penalty. In addition, we also show that intra-rack memory disaggregation would meet the application's memory requirement and provide enough remote memory bandwidth.

==> Cover_letter.tex <==
Dear Editor:

We’re pleased to submit the manuscript entitled ``\textbf{Evaluating the Potential of Disaggregated Memory Systems for HPC applications}'' to be considered for publication in Concurrency and Computation: Practice and Experience.
This is an original submission that has not been published before and that is not currently under review at any other publication outlet. The submission builds on the following conference paper: ``\textbf{N. Ding, S. Williams, H.A. Nam, et al. ``Methodology for Evaluating the Potential of Disaggregated Memory Systems'',2nd International Workshop on RESource DISaggregation in High-Performance Computing (RESDIS), November 18, 2022.}'' 


The current submission extends the previous work in the following ways. We~\textbf{(1) expand our methodology to incorporate the effects of bisection bandwidth on disaggregated memory performance in Section 3.2.} The bisection impact on application performance can be amplified on a disaggregated memory system because users can load data from anywhere in the entire memory pool rather than being confined to a single node. 
We observe that big GEMMs and applications using SuperLU as a preconditioner with 50 solve iterations per factor are sensitive to rack-level disaggregation, while they have no performance penalty with injection bandwidth. Applications using SuperLU with 100 solve iterations per factor will pay the global bisection penalty. Such insights can guide the HPC architects to choose a proper disaggregation level based on their running workloads.
~\textbf{(2) Evaluate the proposed methodology with two new proxy applications --- SuperLU\_DIST and an eigensolver, in Section 5.3.} SuperLU\_DIST and the eigensolver represent two different kinds of traditional HPC workloads. SuperLU\_DIST is a distributed memory sparse direct solver for large sets of linear equations. It factors the system (SpLU) and performs a pair of triangular solves (SpTS) for each of the 100+ iterations of the iterative solver. These two components dominate the run time. The core computation of the eigensolver is sparse matrix-matrix multiplication (SpMM). The performance bound of applications using SuperLU\_DIST as a preconditioner on a disaggregated memory system depends on the number of SpTS per SpLU. While applications which perform computations like the eigensolver will pay the injection bandwidth penalty.
~\textbf{(3) Release of profiling and plotting capabilities.} The repository includes system architecture design space, application performance potentials, and profiling scripts. Readers should be able to apply our methodology and analysis to their own kernels or applications with the scripts and Python 3.10.


The basic findings of the paper and their significance for theory and practice can be summarized as follows. Our methodology for evaluating application performance on disaggregated memory systems allows us to understand the hardware capability and limitations as well as application performance thereby providing insights and guidance to vendors developing technologies that support disaggregated memory.  The unified visualization of local to remote memory access ratio (L:R) and memory capacity endows users with greater insights as to how different aspects of disaggregated memory systems bound performance. HPC system architects could use our methodology to evaluate different disaggregated memory system architectures for their respective workloads (a time- and space-weighted set of applications). 

\vspace{0.5in}
Thank you for your consideration.

\vspace{0.25in}
Sincerely,


Nan Ding



